MedicalAgentsBench for Complex Medical Reasoning: Comparing Internalized Reasoning Models versus Externalized Agent-based Frameworks

Complex medical reasoning requires integrating heterogeneous clinical evidence across multiple inference steps. Large language models (LLMs) now approach this through two routes: internalized reasoning and externalized agent scaffolding (frameworks that decompose problems collaboratively amongst multiple LLMs). To determine whether these routes are exclusive or complementary, we introduce MedicalAgentsBench, a filtered benchmark of 862 complex clinical questions drawn from the union of eight medical datasets via difficulty-aware curation and contamination screening. Evaluating three internalized reasoning models (DeepSeek-R1, o1-mini, and o3-mini), seven base models, and nine externalized agent-based methods, we find that internalized and externalized approaches each independently improve performance, and that their benefits compound: the highest accuracy is achieved by layering agent workflows onto an internalized reasoning model (i.e., o3-mini + MDAgents with 35.1%). Pareto analysis shows this combination dominates the cost-performance frontier; moreover, lightweight optimization on inexpensive models offers an entry point for resource-constrained settings. Our benchmark is at https://github.com/gersteinlab/MedicalAgentsBench.

==> sections/10_figure_legends.tex <==
\section*{MAIN FIGURE TITLES AND LEGENDS}

\setcounter{figure}{0}

\refstepcounter{figure}\label{fig:medagent_teaser_1b}
\noindent\textbf{Figure \thefigure. Performance analysis of large language models on medical tasks.}
Overall \textbf{Pass@1} accuracy comparison across models in zero-shot setting. \danielnew{Hatched bars denote internalized reasoning models.}
The score is \danielnew{averaged over ten evaluation subsets} (MedQA, PubMedQA, MedMCQA, MedBullets, MMLU, MMLU-Pro, \danielnew{AfrimedQA,} MedExQA, and \danielnew{MedXpertQA-R and MedXpertQA-U}).

\bigskip
\refstepcounter{figure}\label{fig:reasoning_depth}
\noindent\textbf{Figure \thefigure. Reasoning depth distribution by dataset split.}
Violin plots comparing the density of reasoning depth ratings (Levels 1--5) between the complete source datasets (Full) and the curated \Ours{} subset (Hard). $\kappa$ values indicate inter-annotator agreement for each domain. Full details of annotation can be found in the human validation protocol in Methods.

\bigskip
\refstepcounter{figure}\label{fig:data_contamination}
\noindent\textbf{Figure \thefigure. Data contamination analysis across medical question-answering datasets using MELD.}
The boxplots display similarity percentages between model-generated text and original question text, with higher values potentially indicating memorization of training data.
Lower similarity scores suggest minimal data contamination, while higher values may indicate potential contamination in model training data.

\bigskip
\refstepcounter{figure}\label{fig:pareto_front}
\noindent\textbf{Figure \thefigure. Cost-performance analysis across medical datasets, comparing open and closed-source language models.}
\danielnew{Each subplot shows the ten base models for one dataset, plotting Pass@1 accuracy (\%) against inference cost per sample (USD, log scale). Circles denote internalized reasoning models and squares denote non-reasoning models; pink markers indicate open-source models and gray markers indicate closed-source models. The red dashed line traces the empirical Pareto frontier, and each subplot title reports the highest-accuracy model for that dataset.}

\bigskip
\refstepcounter{figure}\label{fig:medagent_pareto}
\noindent\textbf{Figure \thefigure. Cost-performance analysis of reasoning methods on \Ours{}.}
Pass@1 accuracy versus inference cost per sample (log scale). Different markers represent reasoning methods; \danielnew{base-model logo colors follow Figure~1;} marker sizes indicate inference time. The red dashed line traces the Pareto frontier of non-dominated configurations. Annotated arrows highlight two distinct mechanisms: \emph{Externalizing} reasoning (adding agent scaffolding to a fixed model) increases both accuracy and cost, while \emph{Internalizing} reasoning (switching to a reasoning model) improves accuracy while reducing inference cost.

\bigskip
\refstepcounter{figure}\label{fig:hardset_pipeline}
\noindent\textbf{Figure \thefigure. Hard-set construction pipeline for \Ours{}.}
Questions are aggregated from eight established medical QA datasets and filtered via a three-stage selection process based on model performance, per-dataset sampling, and reasoning depth.
The resulting set is verified using automated contamination analysis and human validation by M.D. students.
The final benchmark contains 862 curated hard questions, with per-dataset composition shown on the right.

\bigskip
\refstepcounter{figure}\label{fig:answer_correct_distribution}
\noindent\textbf{Figure \thefigure. Distribution of model performance across eight medical datasets.}
MedQA, MedMCQA, PubMedQA, MedBullets, MMLU-Pro, MMLU, MedExQA, and MedXpertQA. Each subplot shows the number of questions answered correctly by different proportions of models (x-axis: k/N, where k is the number of correct models and N is the total number of models). Questions are categorized as either hard (left of the dashed line, $<$ 50\% of models correct) or easy (right of the dashed line, $\geq$ 50\% of models correct), with selected questions highlighted in darker shades. The total question count for each dataset is indicated in the subplot titles.


==> sections/11_main_tables.tex <==
% Main-text table captions only.
% Per Cell Press production requirements, the four main tables are
% uploaded as separate Word files. Captions remain here (analogous to
% figure legends) so that in-text \ref{tab:...} references resolve.

%% ============================================================
%% Table 1: Methods Overview
%% ============================================================
\begin{table}[H]
\caption{\textbf{Methods Overview.} The reasoning approaches span four categories: traditional prompting, advanced prompting, discussion-based agent frameworks, and agentic workflow optimization methods.}
\label{tab:medbench_methods}
\end{table}


%% ============================================================
%% Table 2: Medical Question-Answering Datasets
%% ============================================================
\begin{table}[H]
\caption{\textbf{Medical Question-Answering Datasets.} Benchmarks cover professional medical examinations, biomedical literature and education, and general-domain reasoning tasks with medical content.}
\label{tab:medbench_dataset}
\end{table}


%% ============================================================
%% Table 3: Performance by model and task
%% ============================================================
\begin{table}[H]
\caption{\textbf{Performance by model and task.} Accuracy values are in percentages with standard errors, reported as mean $\pm$ std over 3 runs. The best values are highlighted in \textbf{bold}, and the second-best values are highlighted in \underline{underlined} format.}
\label{tab:model_task_heatmap}
\end{table}


%% ============================================================
%% Table 4: Performance by task and method
%% ============================================================
\begin{table}[H]
\caption{\textbf{Performance by task and method.} All tasks are evaluated on the Hard set. Each model is evaluated separately with all applicable methods. Accuracy values are in percentages, reported as mean $\pm$ std over 3 runs. The best values are highlighted in \textbf{bold}, and the second-best values are highlighted in \underline{underlined} format.}
\label{tab:method_task_heatmap}
\end{table}


==> tables/a3.reason_errors.tex <==
\begin{table*}[hbt!]
\centering
\tiny
\caption{\textbf{Example of reasoning-driven failure.}
The reasoning model, e.g., Deepseek-R1, discovers the correct diagnosis early but, due to overthinking and repeated reconsideration of weaker alternatives, ultimately rejects its strongest evidence and outputs an incorrect answer.
}
\label{tab:medbullets_example_1}
\begin{tabular}{p{0.32\textwidth}p{0.32\textwidth}p{0.32\textwidth}}
\toprule
\multicolumn{3}{p{\linewidth}}{
\textbf{Dataset:} MedBullets \newline
\textbf{Question:} A 55-year-old man presents to the emergency department with nausea and vomiting for the past week. He decided to come in when his symptoms worsened. He feels that his symptoms are exacerbated with large fatty meals and when he drinks alcohol. His wife recently returned from a cruise with symptoms of vomiting and diarrhea. The patient has a medical history of poorly managed diabetes, constipation, anxiety, dyslipidemia, and hypertension. His temperature is 99.5°F (37.5°C), blood pressure is 197/128 mmHg, pulse is 100/min, respirations are 17/min, and oxygen saturation is 95\% on room air. Physical exam reveals a systolic murmur heard loudest along the left upper sternal border. Abdominal exam reveals an obese, tympanitic and distended abdomen with a 3 cm scar in the right lower quadrant. Vascular exam reveals weak pulses in the lower extremities. Which of the following is the most likely underlying etiology of this patient's symptoms?
\newline
\textbf{Options:} A. Adhesions; B. Enteric nervous system damage; C. Impacted stool; D. Norovirus; E. Twisting of the bowel.\newline
\textbf{Correct Answer:} A (Adhesions).\newline
\textbf{Clinical Explanation:} This patient is presenting with abdominal pain and a tympanitic abdomen, which are symptoms suggestive of a small bowel obstruction. In developed countries, these typically occur secondary to adhesions. Small bowel obstructions (SBO) typically present with an absence of bowel sounds, bowel movements, and flatus, as well as abdominal distension, nausea, and vomiting. They typically occur secondary to adhesions which entrap the bowel and disrupt its normal peristalsis. Adhesions can occur after abdominal surgery or trauma as part of the normal healing process. The diagnosis of SBO can be confirmed using abdominal imaging such as a CT scan. Treatment often involves observation; however, surgical decompression of the SBO may be needed if there is a closed-loop obstruction or an obstruction that does not resolve on its own.
} \\
\midrule
\textbf{GPT-4o} & \textbf{o3-mini} & \textbf{DeepSeek-R1} \\
\midrule

A (Correct) &
A (Correct) &
B (Incorrect) \\
\midrule
\textbf{To determine the most likely underlying etiology of this patient's symptoms, let's analyze the information provided step-by-step:}

\textbf{1. Symptoms and History:}
The patient has nausea and vomiting for the past week, worsened by large fatty meals and alcohol. His wife recently had symptoms of vomiting and diarrhea after returning from a cruise, suggesting a possible infectious etiology. The patient has a history of poorly managed diabetes, constipation, anxiety, dyslipidemia, and hypertension.

\textbf{2. Vital Signs:}
Temperature: 99.5°F (37.5°C) - slightly elevated, but not indicative of a high fever. Blood pressure: 197/128 mmHg - significantly elevated, indicating hypertensive urgency. Pulse: 100/min - tachycardia. Respirations: 17/min - normal. Oxygen saturation: 95\% on room air - normal.

\textbf{3. Physical Exam:}
Systolic murmur heard loudest along the left upper sternal border - could indicate aortic stenosis or another cardiac condition. Abdominal exam: obese, tympanitic, and distended abdomen with a 3 cm scar in the right lower quadrant - suggests previous surgery, possibly appendectomy. Vascular exam: weak pulses in the lower extremities - could indicate peripheral artery disease.

\textbf{4. Possible Etiologies:}
\textit{Adhesions (A):} Given the history of abdominal surgery (scar in the right lower quadrant), adhesions could cause bowel obstruction, leading to nausea and vomiting.
\textit{Enteric nervous system damage (B):} This could be related to his poorly managed diabetes, but it is less likely to cause acute symptoms exacerbated by fatty meals and alcohol.
\textit{Impacted stool (C):} Constipation is part of his medical history, but it is less likely to cause acute exacerbation with fatty meals and alcohol.
\textit{Norovirus (D):} The patient's wife had symptoms of vomiting and diarrhea after a cruise, suggesting a possible infectious cause. However, the patient's symptoms are exacerbated by fatty meals and alcohol, which is less typical for norovirus.
\textit{Twisting of the bowel (E):} This could cause acute symptoms of bowel obstruction, but there is no specific mention of acute, severe abdominal pain or signs of peritonitis.

Considering the patient's history of abdominal surgery, the nature of his symptoms, and the physical exam findings, the most likely underlying etiology is \textbf{adhesions} causing bowel obstruction.

Therefore, the correct answer is: \textbf{(A) Adhesions}.
&
\textbf{Step 1: Analyze the patient’s history and examination findings.}

The patient is a 55-year-old man with nausea and vomiting for a week. His symptoms worsen with fatty meals and alcohol. There is a notable 3 cm scar in the right lower quadrant, suggesting prior abdominal surgery. His exam reveals an obese, tympanitic, and distended abdomen.

\textbf{Step 2: Consider possible causes based on the provided options.}

\textit{(A) Adhesions:} After any abdominal surgery, adhesions can form. These are the most common cause of small bowel obstruction, which can present with nausea, vomiting, and abdominal distension.

\textit{(B) Enteric nervous system damage:} This could be related to diabetic gastroparesis. However, gastroparesis typically does not cause a tympanitic, distended abdomen, and a surgical scar points away from this diagnosis.

\textit{(C) Impacted stool:} While the patient has a history of constipation, impacted stool usually does not lead to prolonged vomiting over a week and a distended, tympanitic abdomen.

\textit{(D) Norovirus:} Although the wife had gastrointestinal symptoms from a recent cruise, a norovirus infection generally causes acute diarrhea and vomiting rather than a week-long picture with abdominal distension.

\textit{(E) Twisting of the bowel (volvulus):} This can cause obstruction, but it is more often seen in the context of malrotation or specific colonic volvulus and less likely with a history of prior abdominal surgery evident from the scar.

\textbf{Step 3: Correlate the findings.}

The presence of a previous surgical scar in the right lower quadrant (likely from an appendectomy) combined with the abdominal distension and vomiting strongly supports the diagnosis of a small bowel obstruction due to postoperative adhesions.

\textbf{Final Answer:} A.
&
\textbf{<think>}

Okay, let's try to work through this question step by step. The patient is a 55-year-old man with a week of nausea and vomiting that's worse after fatty meals and alcohol. His wife had vomiting and diarrhea from a cruise, which makes me think of possible infections like norovirus. But his other symptoms might point elsewhere.

His medical history includes poorly managed diabetes, which can lead to complications like gastroparesis due to autonomic neuropathy (enteric nervous system damage). ...

The systolic murmur along the left upper sternal border—maybe aortic stenosis? Or another heart issue. But the main issue here is the GI symptoms. Let's think about the possible causes of his nausea and vomiting exacerbated by fatty meals. That's classic for biliary issues like cholecystitis, but the question is about the underlying etiology. However, the options given don't include that. The options are adhesions, enteric nervous system damage (like gastroparesis), impacted stool, norovirus, or twisting (volvulus).

His wife's norovirus could be a red herring. He has risk factors for gastroparesis (diabetes), which causes delayed gastric emptying. Symptoms of gastroparesis include nausea, vomiting, especially after meals high in fat or fiber. Alcohol can also exacerbate it. The distended abdomen might be from delayed emptying. But then there's the tympanitic abdomen, which could be from gas due to obstruction or ileus.

He has a history of constipation. Impacted stool (option C) could lead to obstruction, causing nausea and vomiting, but the exacerbation with fatty meals and alcohol seems more like a motility issue. Adhesions (A) from prior surgery (the scar) could cause mechanical obstruction. But the presentation here isn't acute; it's been a week. Volvulus (E) would present more acutely with severe pain.

Diabetic gastroparesis (B) fits with the diabetes history and the triggers. The autonomic neuropathy damages the enteric nerves, leading to poor motility. The distended abdomen could be from gastric distension. The tympany might be from gas in the stomach.

\hlc{pink!60}{But wait, the abdominal exam says "distended and tympanitic," which is more suggestive of an ileus or obstruction. If it's an ileus, that's a motility problem.} Diabetic autonomic neuropathy can cause ileus. Impacted stool (C) would present with constipation and possible obstruction. But he's had constipation as part of his history. However, the exacerbation with fatty meals and alcohol points more towards gastroparesis.

\hlc{pink!60}{Alternatively, the high blood pressure and weak pulses in the legs could indicate atherosclerosis, maybe mesenteric ischemia, but that's not one of the options. The options given are A to E.}

So, the options again: A) Adhesions, B) Enteric nervous system damage, C) Impacted stool, D) Norovirus, E) Twisting.

The wife's norovirus (D) could be a coincidental exposure, but his symptoms are more chronic (a week) and not primarily diarrhea. His symptoms are more upper GI (nausea, vomiting) and related to meals.

\hlc{teal!20}{Adhesions (A) from prior surgery (scar in RLQ) could cause a small bowel obstruction.} Symptoms of obstruction include nausea, vomiting, distention, and tympanitic abdomen. \hlc{pink!60}{But the exacerbation with fatty meals and alcohol isn't typical for obstruction. However, if the obstruction is partial, maybe certain foods make it worse.} ...

\hlc{pink!60}{But the patient's history of diabetes and the triggers (fatty meals, alcohol) might still point more towards gastroparesis (B).} ...

Impacted stool (C) would present with constipation and possible obstipation. If he's been constipated and has a history of it, maybe fecal impaction leading to obstruction. But the exacerbation with meals might not directly relate.

So, the key factors here are the triggers (fatty meals, alcohol) and the diabetes. \hlc{pink!60}{Diabetic gastroparesis is a likely candidate.} So the underlying etiology would be enteric nervous system damage (B).

\hlc{pink!60}{But wait, the physical exam shows a distended and tympanitic abdomen. In gastroparesis, the stomach may be distended, but the tympany could be from that. However, if there's an ileus, that's also a motility issue. But the question is about the underlying cause. The diabetes leading to autonomic neuropathy (enteric nervous system damage) would be the etiology.}

\textbf{\hlc{pink!60}{So the answer is B.}}

\textbf{</think>}
\\
\bottomrule
\end{tabular}
\end{table*}

==> tables/a4.small_model_error.tex <==
\begin{table*}[hbt!]
\centering
\tiny
\caption{\textbf{Example of reasoning-driven success.}
The reasoning model, e.g., Deepseek-R1, considers worsening symptoms in context, resists premature treatment changes, and maintains the strongest evidence, avoiding overreaction and producing the correct answer.
}
\label{tab:medbullets_example_2}
\begin{tabular}{p{0.32\textwidth}p{0.32\textwidth}p{0.32\textwidth}}
\toprule
\multicolumn{3}{p{\linewidth}}{
\textbf{Dataset:} MedBullets \newline
\textbf{Question:} A 31-year-old man presents with fever, malaise, cough, and hemoptysis. He was previously diagnosed with HIV (CD4 40/mm\textsuperscript{3}, viral load 115{,}000 copies/mL) and treated for a right upper lobe infiltrate. After 4 weeks on ART, his CD4 rose to >400/mm\textsuperscript{3} and viral load became negligible. Now he presents with new left upper lobe nodules and hilar adenopathy on chest radiograph. What is the most appropriate next step in management? \newline
\textbf{Options:} A. Continue current anti-retroviral treatment, antimicrobial, and anti-tuberculoid therapies; B. Determine drug sensitivities; C. Discontinue antimicrobial treatment; D. Obtain a D-dimer; E. Start high-dose glucocorticoid treatment and discontinue antiretroviral therapy. \newline
\textbf{Correct Answer:} A (Continue current therapies). \newline
\textbf{Clinical Explanation:} This patient with recently diagnosed HIV and tuberculosis infection (upper lung lobe infiltrate) is presenting with worsening symptoms after being appropriately treated. Worsening of symptoms after initiation of these therapies is concerning for immune reconstitution inflammatory syndrome (IRIS), which is managed by continuing current combined antiretroviral medications, antibiotics for opportunistic infections and symptom management. IRIS describes a paradoxical worsening of a patient's underlying infection after initiating antiretroviral therapy for patients with HIV. IRIS can also occur in HIV-uninfected patients with tuberculosis or leprosy who are started on antimycobacterial treatment. The pathogenesis of IRIS is unclear, but in patients with HIV, antiretroviral therapy increases the amount of CD4+ T-helper cells, which can lead to an exaggerated inflammatory response (e.g., increased cytokine release) towards the infection. Thus, there is a paradoxical worsening of the infection symptoms. When patients have a paradoxical worsening of their symptoms in the setting of starting their antiretroviral therapy, the therapy should be continued with symptomatic management (acetaminophen for fever). Nelson et al review IRIS. They note it is seen in patients with HIV. They recommend antiretroviral therapy and antibiotics for bacterial infections.
} \\
\midrule
\textbf{GPT-4o-mini} & \textbf{GPT-4o} & \textbf{DeepSeek-R1} \\
\midrule

B (Incorrect) &
E (Incorrect) &
A (correct) \\
\midrule
To approach this clinical scenario, we need to analyze the patient's presentation and history step-by-step:

1. \textbf{Patient Background}: The patient is a 31-year-old man with a history of HIV, presenting with fever, malaise, cough, and hemoptysis (blood in sputum). He has a very low CD4 count (40/mm\textsuperscript{3}) and a high HIV viral load (115,000 copies/mL) at the time of his previous visit.

2. \textbf{Previous Treatment}: He was treated for a right upper lobe lung infiltrate, which suggests a possible opportunistic infection, common in patients with low CD4 counts. After treatment, his CD4 count improved significantly to over 400/mm\textsuperscript{3}, and his HIV viral load became negligible.

3. \textbf{Current Symptoms}: The patient now presents with worsening cough, fever, and new findings on chest radiograph, which shows new nodules in the left upper lobe and hilar adenopathy. This raises concern for a possible new pulmonary infection or a reactivation of a previous infection, especially given his history of low CD4 count.

4. \textbf{Differential Diagnosis}: Given the patient's immunocompromised state, the differential diagnosis could include:
   - Tuberculosis
   - Fungal infections
   - Bacterial pneumonia
   - Lymphoma or other malignancies

5. \textbf{Next Steps in Management:} 
\hlc{pink!60}{The most appropriate next step in management would be to determine the cause of the new pulmonary findings. This could involve obtaining cultures or sensitivities to identify the specific pathogen responsible for the patient's symptoms.}

\textbf{Now, let's evaluate the options:}  

\hlc{pink!60}{(A) Continuing current treatments without further investigation may not address the new findings.}

\hlc{pink!60}{(B) Determining drug sensitivities against the patient’s pulmonary infection is crucial to guide appropriate treatment.}

(C) Discontinuing antimicrobial treatment is not advisable given the new symptoms.  

(D) Obtaining a D-dimer level is not relevant in this context.  

(E) Starting high-dose glucocorticoid treatment and discontinuing antiretroviral therapy is inappropriate.

Based on this analysis, the most appropriate next step in management is:  
\textbf{B) Determine drug sensitivities against the patient’s pulmonary infection.}
&

To determine the most appropriate next step in management for this patient, let's analyze the clinical scenario step-by-step:

1. \textbf{Patient History and Symptoms}: 
- 31-year-old HIV-positive man with fever, malaise, hemoptysis  
- prior CD4 40/mm\textsuperscript{3}, high viral load  
- after treatment, CD4 >400/mm\textsuperscript{3}, viral load negligible  

2. \textbf{Current Presentation}: 
- Fever 102°F  
- Nodules in left upper lobe  
- Hilar adenopathy  

3. \textbf{Possible Diagnoses}:  
\hlc{pink!60}{Given the patient's history of HIV and recent improvement in CD4 count, the new pulmonary findings could suggest an immune reconstitution inflammatory syndrome (IRIS).}  
\hlc{pink!60}{The presence of new nodules and hilar adenopathy could indicate a reactivation or worsening of a previous infection.}

4. \textbf{Management Considerations}:  
\hlc{pink!60}{Continuing current treatments (Option A) might not address the new findings adequately.}  
\hlc{pink!60}{Determining drug sensitivities (Option B) could be useful if there is suspicion of drug-resistant infection.}  
\hlc{pink!60}{Starting high-dose glucocorticoid treatment and discontinuing antiretroviral therapy (Option E) could be considered if IRIS is strongly suspected.}

\hlc{pink!60}{Given the clinical context and the likelihood of IRIS, the most appropriate next step is to manage the inflammatory response while continuing to treat the underlying HIV infection. Therefore, the best option is:  
\textbf{(E) Start high-dose glucocorticoid treatment and discontinue antiretroviral therapy.}}

\hlc{pink!60}{This approach addresses the potential IRIS by reducing inflammation and temporarily halting the immune reconstitution that may be exacerbating the symptoms.}
&

\textbf{<think>}

Okay, let's tackle this question. So, the patient is a 31-year-old man with a history of HIV. He was treated for a lung infiltrate 5 weeks ago, and his CD4 count went up after treatment. Now he's back with worsening symptoms, new nodules on the chest X-ray, and hilar adenopathy.

First, I need to recall what happens when someone with HIV starts antiretroviral therapy (ART). When they start ART, especially if they had a very low CD4 count (like 40 here), there's a risk of immune reconstitution inflammatory syndrome (IRIS). IRIS occurs when the immune system starts recovering and mounts an exaggerated response to an existing infection, causing inflammation. This can make existing infections worse or cause new symptoms even if the infection was being treated.

His previous treatment probably included antibiotics for the lung infiltrate. Now, after starting ART, his CD4 count improved (from 40 to over 400), which is a good response. But now he's presenting with new nodules and adenopathy. The timing (4 weeks after starting ART) fits with IRIS. The new nodules could be a paradoxical reaction to the treatment of an infection, like tuberculosis or another opportunistic infection. Since he was treated before and now has new findings, maybe the initial infection is still present, and the immune system is reacting to it more now.

Looking at the options: 

A) Continue current treatments. If it's IRIS, continuing ART and antimicrobials is correct, but maybe add something else? But the options don't mention adding steroids here. Wait, option E says start glucocorticoids and stop ART. But stopping ART is not recommended.

\textbf{So the best answer is A.}

\textbf{</think>}
\\
\bottomrule
\end{tabular}
\end{table*}

==> tables/a5.iterative_error.tex <==
\begin{table*}[hbt!]
\centering
\tiny
\caption{\textbf{Example of reasoning-driven self-correction.}
Self-Refine reliably overturns an initial incorrect hypothesis through iterative reevaluation, while MultiPersona reasoning amplifies early biases across agents and may even suppress emerging correct reasoning signals.}
\label{tab:medbullets_example_3}
\begin{tabular}{p{0.32\linewidth}p{0.32\linewidth}p{0.32\linewidth}}
\toprule
\multicolumn{3}{p{\linewidth}}{
\textbf{Dataset:} MedBullets \newline
\textbf{Question:} A 5-year-old girl presents to the emergency room due to difficulty walking. She has been complaining of pain in her right leg for the last few days. Her neighbor’s cat bit her last week and her parents attributed the pain to her healing bite. At the time of the bite, they cleaned the wound and irrigated it with sterile saline water from a first aid kit. She has no medical history and has never been hospitalized. Her temperature is 102.2°F (39°C), blood pressure is 118/78 mmHg, pulse is 90/min, respirations are 21/min, and pulse oximetry is 99\% on room air. The open wound remains present on the thigh with surrounding erythema and edema. MRI is consistent with osteomyelitis. Which of the following is the most appropriate next step in management?  \newline
\textbf{Options:} A. Amoxicillin and clavulanate; B. Ampicillin and sulbactam; C. Doxycycline; D. Fluconazole; E. Vancomycin. \newline
\textbf{Correct Answer:} B (Ampicillin and sulbactam). \newline
\textbf{Clinical Explanation:} This young girl with a recent history of a cat bite and difficulty walking most likely has likely Pasteurella multocida osteomyelitis. Empiric IV antibiotic therapy with ampicillin-sulbactam is the most appropriate initial management. Pasteurella multocida is a gram-negative rod that is associated with cat and dog bites. Infection can lead to cellulitis and osteomyelitis. Treatment of minor infection is with amoxicillin-clavulanate; however, patients suspected of having osteomyelitis should be treated empirically with IV antibiotics (e.g., ampicillin and sulbactam) and taken for biopsy/culture to identify the pathogen. Antibiotics can then be narrowed down accordingly. Patients will often require between 4-8 weeks of antibiotic treatment. MRSA coverage may initially be started and tapered later once cultures result. Mollitt reviews the evidence regarding the microbiology of various injuries. He discusses how Pasteurella multocida is a common complication of animal bites. He recommends early effective antibiotic treatment.
} \\
\midrule
\multicolumn{3}{p{\linewidth}}{
\textbf{Chain-of-Thought:} E (Incorrect)} \\
\multicolumn{3}{p{\linewidth}}{
To determine the most appropriate next step in management for this 5-year-old girl presenting with symptoms consistent with osteomyelitis, let's analyze the situation step-by-step:

1. \textbf{Patient Presentation}:  
The girl has difficulty walking and pain in her right leg, which started a few days after a cat bite. The wound is still open with surrounding erythema and edema, and she has a fever (102.2°F).

2. \textbf{Vital Signs}:  
Her vital signs show a fever, but her blood pressure, pulse, respirations, and oxygen saturation are within normal limits for her age.

3. \textbf{Diagnosis}:  
The MRI confirms osteomyelitis, which is an infection of the bone. This condition can occur following a penetrating injury, such as a cat bite, especially if the wound becomes infected.

4. \textbf{Common Pathogens}:  
Cat bites can introduce various bacteria, including \textit{Pasteurella multocida}, \textit{Staphylococcus aureus}, and \textit{Streptococcus} species. Osteomyelitis in children is often caused by \textit{Staphylococcus aureus}, including methicillin-resistant \textit{Staphylococcus aureus} (MRSA).

5. \textbf{Antibiotic Choice}:  
The treatment for osteomyelitis typically involves antibiotics that cover the most likely pathogens.  
\hlc{pink!60}{Given the possibility of MRSA and the severity of the infection, the reasoning incorrectly prioritizes MRSA coverage over Pasteurella coverage.}

6. \textbf{Options Analysis}:  
- \textbf{Amoxicillin and clavulanate (A)}: Effective against many bacteria, including \textit{Pasteurella multocida}, but not the best choice for MRSA.  
- \textbf{Ampicillin and sulbactam (B)}: Effective against many bacteria but not the best choice for MRSA.  
- \textbf{Doxycycline (C)}: Can treat MRSA, but not first-line in children with severe infections.  
- \textbf{Fluconazole (D)}: Antifungal; not appropriate.  
- \textbf{Vancomycin (E)}: Effective against MRSA.  

\hlc{pink!60}{Given the need to cover MRSA and the severity of the infection, the model incorrectly concludes that the most appropriate next step is vancomycin.}

\textbf{Final Answer:}  
\hlc{pink!60}{(E) Vancomycin}
}\\
\midrule
\textbf{Self-Refine | Round 1:} A (Incorrect) & \textbf{Round 2:} B (Correct) & \textbf{Round 3:} B (Correct) \\
To determine the most appropriate next step in management for this 5-year-old girl presenting with osteomyelitis following a cat bite, let's analyze the situation step by step:\newline
1. \textbf{Patient Presentation}: The girl has difficulty walking, pain in her right leg, and a history of a cat bite. She has a fever (102.2°F), and the wound shows signs of infection (erythema and edema).\newline
2. \textbf{Diagnosis}: MRI confirms osteomyelitis, which is an infection of the bone.\newline
3. \textbf{Likely Pathogens}: Cat bites can introduce various bacteria, including Pasteurella multocida, Staphylococcus aureus, and Streptococcus species. Pasteurella multocida is particularly common in cat bites.\newline
4. \textbf{Antibiotic Choice}:
- \textbf{Amoxicillin and clavulanate (A)}: Effective against Pasteurella multocida and other common pathogens in cat bites.
- \textbf{Ampicillin and sulbactam (B)}: Also effective against Pasteurella multocida and other common pathogens.
- \textbf{Doxycycline (C)}: Effective against Pasteurella multocida but not typically first-line in young children due to potential side effects on teeth and bones.
- \textbf{Fluconazole (D)}: An antifungal, not appropriate for bacterial osteomyelitis.
- \textbf{Vancomycin (E)}: Effective against MRSA and other Gram-positive bacteria but not the first choice for Pasteurella multocida.\newline
5. \textbf{Considerations}:
- The patient is a child, so the antibiotic should be safe for pediatric use.
- The antibiotic should cover Pasteurella multocida and other common pathogens from cat bites.
\hlc{pink!60}{Given these considerations, the most appropriate next step in management is to choose an antibiotic that is effective against the likely pathogens and safe for pediatric use.}\newline
\hlc{pink!60}{Both amoxicillin and clavulanate (A) and ampicillin and sulbactam (B) are suitable choices, but amoxicillin and clavulanate is more commonly used in outpatient settings and is a well-known first-line treatment for cat bites.}\newline
Therefore, the most appropriate next step in management is:
\textbf{(A) Amoxicillin and clavulanate}
&
\textbf{Review response}:
True. The solution provided is correct. Here is a step-by-step reasoning to confirm the correctness:\newline

... [Same as Round 1]\newline

The solution correctly identifies the appropriate antibiotic for treating osteomyelitis following a cat bite in a pediatric patient.\newline
\textbf{Revised response}:
To revise the solution for the given problem, let's ensure we follow the correct steps and address the feedback appropriately.\newline
1. \textbf{Patient Presentation}: The 5-year-old girl has difficulty walking, pain in her right leg, and a history of a cat bite. She has a fever (102.2°F), and the wound shows signs of infection (erythema and edema).\newline
2. \textbf{Diagnosis}: MRI confirms osteomyelitis, which is an infection of the bone.\newline
3. \textbf{Likely Pathogens}: Cat bites can introduce various bacteria, including Pasteurella multocida, Staphylococcus aureus, and Streptococcus species. Pasteurella multocida is particularly common in cat bites.\newline
4. \textbf{Antibiotic Choice}:
- \textbf{Amoxicillin and clavulanate (A)}: Effective against Pasteurella multocida and other common pathogens in cat bites.
- \textbf{Ampicillin and sulbactam (B)}: Also effective against Pasteurella multocida and other common pathogens.
- \textbf{Doxycycline (C)}: Effective against Pasteurella multocida but not typically first-line in young children due to potential side effects on teeth and bones.
- \textbf{Fluconazole (D)}: An antifungal, not appropriate for bacterial osteomyelitis.
- \textbf{Vancomycin (E)}: Effective against MRSA and other Gram-positive bacteria but not the first choice for Pasteurella multocida.\newline
5. \textbf{Considerations}:
- The patient is a child, so the antibiotic should be safe for pediatric use.
- The antibiotic should cover Pasteurella multocida and other common pathogens from cat bites.
\hlc{teal!20}{Given these considerations, the most appropriate next step in management is to choose an antibiotic that is effective against the likely pathogens and safe for pediatric use.}\newline
\hlc{teal!20}{Both amoxicillin and clavulanate (A) and ampicillin and sulbactam (B) are suitable choices, but ampicillin and sulbactam is more commonly used in inpatient settings and is a well-known first-line treatment for osteomyelitis.}\newline
Therefore, the most appropriate next step in management is:
\textbf{(B) Ampicillin and sulbactam}
&

\textbf{Review response}:
The solution provided for the given problem is correct. Here is the step-by-step reasoning:\newline

... [Same as Round 1]\newline

The solution is correct.\newline
\textbf{Revised response}:
To revise the solution for the given problem, let's ensure we follow the correct steps and address the feedback appropriately.\newline
1. \textbf{Patient Presentation}: The 5-year-old girl has difficulty walking, pain in her right leg, and a history of a cat bite. She has a fever (102.2°F), and the wound shows signs of infection (erythema and edema).\newline
2. \textbf{Diagnosis}: MRI confirms osteomyelitis, which is an infection of the bone.\newline
3. \textbf{Likely Pathogens}: Cat bites can introduce various bacteria, including Pasteurella multocida, Staphylococcus aureus, and Streptococcus species. Pasteurella multocida is particularly common in cat bites.\newline
4. \textbf{Antibiotic Choice}:
- \textbf{Amoxicillin and clavulanate (A)}: Effective against Pasteurella multocida and other common pathogens in cat bites.
- \textbf{Ampicillin and sulbactam (B)}: Also effective against Pasteurella multocida and other common pathogens.
- \textbf{Doxycycline (C)}: Effective against Pasteurella multocida but not typically first-line in young children due to potential side effects on teeth and bones.
- \textbf{Fluconazole (D)}: An antifungal, not appropriate for bacterial osteomyelitis.
- \textbf{Vancomycin (E)}: Effective against MRSA and other Gram-positive bacteria but not the first choice for Pasteurella multocida.\newline
5. \textbf{Considerations}:
- The patient is a child, so the antibiotic should be safe for pediatric use.
- The antibiotic should cover Pasteurella multocida and other common pathogens from cat bites.
\hlc{teal!20}{Given these considerations, the most appropriate next step in management is to choose an antibiotic that is effective against the likely pathogens and safe for pediatric use.}
\hlc{teal!20}{Both amoxicillin and clavulanate (A) and ampicillin and sulbactam (B) are suitable choices, but ampicillin and sulbactam is more commonly used in inpatient settings and is a well-known first-line treatment for osteomyelitis.}\newline
Therefore, the most appropriate next step in management is:
\textbf{(B) Ampicillin and sulbactam}
\\
\midrule
\textbf{MultiPersona | Round 1:} E, B, E & \textbf{Round 2:} E, E, E & \textbf{Final:} E (Incorrect) \\
- \textbf{Persona 1 (MD Student):} \hlc{pink!60}{Given the severity of the infection (osteomyelitis) and the need to cover both common pathogens from cat bites and potential MRSA, the most appropriate antibiotic should be broad-spectrum and effective against MRSA. Vancomycin is effective against MRSA, which is a common cause of osteomyelitis in children.}\newline
- \textbf{Persona 2 (Medical Professor):} \hlc{teal!20}{The text outlines the patient's symptoms and the clinical diagnosis of osteomyelitis resulting from a cat bite. It discusses various treatment options, highlighting the necessity for a broad-spectrum antibiotic that can address the common pathogens associated with cat bites, particularly in severe infections. Among the treatment options listed, Ampicillin and sulbactam is noted as effective against many relevant bacteria, making it the most suitable choice for this patient's condition.}\newline
- \textbf{Persona 3 (Medical Researcher):} \hlc{pink!60}{Given the patient's symptoms of osteomyelitis likely caused by a cat bite and the need to cover MRSA, the best antibiotic choice is one that effectively treats these severe infections. Vancomycin is specifically noted for its efficacy against MRSA and other relevant bacteria, making it the most suitable option despite the other available choices not sufficiently covering MRSA or not being appropriate for the situation.}
&
- \textbf{Persona 1 (MD Student):}  \hlc{pink!60}{The patient presents with symptoms consistent with a severe infection, specifically osteomyelitis after a cat bite, which raises the concern for MRSA. Given that vancomycin effectively covers MRSA—a crucial factor due to the severity of the infection—this makes it the most appropriate choice for management. Other antibiotics discussed do not provide coverage for MRSA, making them less suitable in this scenario.}\newline
- \textbf{Persona 2 (Medical Professor):} \hlc{pink!60}{The patient with signs of osteomyelitis and a recent cat bite requires antibiotic treatment. The analysis shows that the infection could be due to MRSA, which is common in such cases. Reviewing the treatment options, vancomycin is identified as the only antibiotic effective against MRSA and suitable for severe infections like osteomyelitis. Therefore, vancomycin is determined to be the most appropriate choice.}\newline
- \textbf{Persona 3 (Medical Researcher):} \hlc{pink!60}{The patient's condition is severe due to osteomyelitis likely caused by a cat bite, thus requiring an antibiotic that covers MRSA and potential polymicrobial infections. Vancomycin is specifically noted for its effectiveness against MRSA and its common use in severe infections like osteomyelitis. Other options do not provide adequate coverage compared to Vancomycin.}
&
\textbf{Final Thinking}\newline
\hlc{pink!60}{The case involves a 5-year-old girl displaying severe infection symptoms following a cat bite, indicating a strong suspicion for MRSA involvement. The evaluation of antibiotic options reveals that only vancomycin effectively targets MRSA, which is critical given the high risk of severe bacterial infection indicated by her clinical presentation and MRI findings. Thus, vancomycin is determined to be the most appropriate choice for treatment.}
\\
\bottomrule
\end{tabular}
\end{table*}

==> tables/a6.multiagent_iterative.tex <==
\begin{table*}[hbt!]
\centering
\tiny
\caption{\textbf{Example of reasoning-driven multi-agent correction.}
Here, multiple personas make early mistakes, yet the multi-persona framework reveals distinct correct rationales and resolves conflicts through consensus. This shows how structured aggregation reduces individual reasoning errors.
}
\label{tab:medbullets_example_4}
\begin{tabular}{p{0.32\linewidth}p{0.32\linewidth}p{0.32\linewidth}}
\toprule
\multicolumn{3}{p{\linewidth}}{
\textbf{Dataset:} MedBullets \newline
\textbf{Question:}
A 43-year-old man presents to the emergency department acutely with altered mental status. He uses intravenous drugs and is unable to offer a history. He was found unconscious in a park. His temperature is 99.0°F (37.2°C), blood pressure is 80/40 mmHg, pulse is 156/min, and respirations are 26/min. Physical exam reveals an obtunded man covered in vomit, with track marks on his arm and several skin abscesses. The patient is given 4 liters of Ringer lactate and intravenous antibiotics. As the fourth liter of fluids is finishing, the patient is noted to have jugular venous distension and an oxygen saturation of 92\% on nonrebreather. He is subsequently intubated. The patient is started on norepinephrine, and his blood pressure is subsequently found to be 85/44 mmHg. Which of the following is the most appropriate next step in management?
\newline
\textbf{Options:} A. Cardioversion; B. Epinephrine; C. Hydrocortisone; D. Normal saline; E. Phenylephrine
\newline
\textbf{Correct Answer:} B (Epinephrine)
\newline
\textbf{Clinical Explanation:} This patient who uses intravenous drugs with skin abscesses (the likely source of his infection) is hypotensive and tachycardic, with a blood pressure that is not responding to IV fluids; this is concerning for septic shock. Given his persistent hypotension, he should be started on vasopressors of which norepinephrine is first line and epinephrine is second line. Septic shock is a life-threatening, systemic bacterial infection that leads to vasodilation and endothelial dysfunction. Early management is centered on IV fluids, blood cultures, broad-spectrum antibiotics, and workup to uncover the source. If the patient's blood pressure does not respond to IV fluids (by definition, their blood pressure will not respond to fluids in septic shock), vasopressors should be started with a goal mean arterial pressure > 65 mmHg. The first line vasopressor is norepinephrine, which can be titrated up for maximal effect. If this vasopressor fails to reach blood pressure goals, then the next vasopressor is either vasopressin or epinephrine (either is acceptable). If the second line vasopressor fails to increase blood pressure, then the third line vasopressor is vasopressin or epinephrine (whichever was not used as the second line pressor). Finally, the fourth line vasopressor for septic shock is phenylephrine. Levy et al. review sepsis. They update the Surviving Sepsis campaign which gives the most up to date management guidelines of sepsis including adequate fluid resuscitation, broad-spectrum antibiotics, and vasopressors. They recommend early antibiotics and resuscitation to minimize morbidity and mortality.
} \\
\midrule
\multicolumn{3}{p{\linewidth}}{
\textbf{Chain-of-Thought:} C (Incorrect)} \\
\multicolumn{3}{p{\linewidth}}{
To determine the most appropriate next step in the management of this patient, let's analyze the situation step-by-step:\newline
1. \textbf{Patient Presentation}: The patient is a 43-year-old man with a history of intravenous drug use, presenting with altered mental status, hypotension, tachycardia, and respiratory distress. He was found unconscious and is now obtunded.\newline
2. \textbf{Vital Signs}:
- Temperature: 99.0°F (37.2°C)
- Blood Pressure: 80/40 mmHg initially, 85/44 mmHg after norepinephrine
- Pulse: 156/min
- Respirations: 26/min
- Oxygen Saturation: 92\% on nonrebreather\newline
3. \textbf{Physical Exam}: The patient has track marks and skin abscesses, indicating intravenous drug use. He is covered in vomit and is obtunded.\newline
4. \textbf{Initial Management}: The patient received 4 liters of Ringer lactate and intravenous antibiotics. Despite fluid resuscitation, he developed jugular venous distension and required intubation.\newline
5. \textbf{Current Status}: After intubation and starting norepinephrine, his blood pressure is still low (85/44 mmHg), and he has jugular venous distension, which suggests fluid overload or cardiac dysfunction.\newline
6. \textbf{ECG Findings}: The ECG (not provided here, but assuming it shows signs of tachycardia and possibly other abnormalities) needs to be considered in the context of the patient's clinical picture.\newline
7. \textbf{Differential Diagnosis}: The patient likely has septic shock given his history of intravenous drug use, skin abscesses, and response to antibiotics. The persistent hypotension despite fluids and norepinephrine suggests refractory septic shock or another underlying issue such as adrenal insufficiency.\newline
8. \textbf{Management Options}:\newline
- (A) Cardioversion: Typically used for arrhythmias like atrial fibrillation or ventricular tachycardia, not indicated here without specific arrhythmia evidence.
- (B) Epinephrine: Another vasopressor that could be considered, but the patient is already on norepinephrine.
- (C) Hydrocortisone: Used in septic shock, especially if adrenal insufficiency is suspected.
- (D) Normal saline: Additional fluids might worsen jugular venous distension and fluid overload.
- (E) Phenylephrine: Another vasopressor, but norepinephrine is already being used.\newline
\hlc{pink!60}{Given the patient's refractory hypotension despite fluids and norepinephrine, and the clinical suspicion of septic shock with possible adrenal insufficiency, the most appropriate next step is:}\newline
\hlc{pink!60}{(C) Hydrocortisone}\newline
\hlc{pink!60}{Hydrocortisone can help in cases of septic shock, particularly if there is adrenal insufficiency, which is a concern in this patient given his refractory hypotension.}\newline
Thus, the answer is (C) Hydrocortisone.
}\\
\midrule
\textbf{MultiPersona | Round 1:} C, C, B & \textbf{Round 2:} B, B, C & \textbf{Final:} B (Correct) \\
- \textbf{Persona 1 (MD Student):} \hlc{pink!60}{The patient's persistent hypotension despite norepinephrine and the presence of signs indicating fluid overload suggests that there may be adrenal insufficiency or refractory septic shock at play. Hydrocortisone is indicated in such situations as it can help address potential relative adrenal insufficiency during septic shock. Therefore, it is the most appropriate next step in management.}\newline
- \textbf{Persona 2 (Medical Professor):} 
\hlc{pink!60}{The patient is not responding adequately to fluids and norepinephrine, suggesting the possibility of adrenal insufficiency in septic shock. Hydrocortisone is appropriate for patients in septic shock who are not adequately responding to other treatments.}\newline
- \textbf{Persona 3 (Medical Researcher):} \hlc{teal!20}{Analyzing the clinical scenario, it is clear that the patient is in septic shock with persistent hypotension despite the initial treatment with fluids and norepinephrine. The options were evaluated, and while several medications were considered, epinephrine is specifically indicated for septic shock when there is inadequate response to norepinephrine. It can enhance cardiac output and systemic vascular resistance, making it the most appropriate next step in this case.}
&
- \textbf{Persona 1 (MD Student):}  
\hlc{teal!20}{The patient is experiencing refractory septic shock with persistent hypotension despite fluid resuscitation and norepinephrine. The recommendation is to use epinephrine as it can improve cardiac output and vascular resistance, which is necessary to stabilize the patient's condition.}\newline
- \textbf{Persona 2 (Medical Professor):} \hlc{teal!20}{Given the patient's persistent hypotension despite norepinephrine administration, epinephrine is identified as a reasonable next step since it enhances cardiac output and systemic vascular resistance, which is crucial in managing refractory septic shock. It is regarded as the most appropriate option for stabilization in this scenario.}\newline
- \textbf{Persona 3 (Medical Researcher):} \hlc{pink!60}{The patient presents with refractory hypotension despite fluid resuscitation and vasopressor therapy. This suggests a potential adrenal insufficiency in the context of septic shock, which requires treatment with hydrocortisone. Other options do not align with the management of the current clinical scenario.}
&
\textbf{Final Thinking}\newline
\hlc{teal!20}{The patient is in refractory septic shock with persistent hypotension despite fluid resuscitation and norepinephrine administration, indicating that initial treatment is ineffective. Given the options, epinephrine stands out as the most appropriate next step because it provides both vasopressor and inotropic support, which is crucial for stabilizing the hemodynamics in this scenario.}
\\
\bottomrule
\end{tabular}
\end{table*}

==> tables/a7.multiagent_errors.tex <==
\begin{table*}[hbt!]
\centering
\tiny
\caption{\textbf{Example of MedAgents consensus-driven correction.}
Unlike naive multi-agent voting, which amplifies shared biases, MedAgents employs domain decomposition, synthesis, and cross-expert verification to identify and correct reasoning faults. Disagreements trigger revisions, enabling iterative refinement toward more reliable, clinically aligned answers.
}
\label{tab:medbullets_example_5}
\begin{tabular}{p{0.32\linewidth}p{0.32\linewidth}p{0.32\linewidth}}
\toprule
\multicolumn{3}{p{\linewidth}}{
\textbf{Dataset:} MedBullets \newline
\textbf{Question:} 
A 4-week-old boy is brought to the pediatrician by his parents for an initial evaluation. His parents are concerned that he is not feeding well and has lost weight over the last 2 weeks. He was born at home via spontaneous vaginal delivery at 37 weeks of gestation to a G1P1 mother. His mother did not receive prenatal care. His blood pressure is 70/44 mmHg, pulse is 151/min, and respirations are 41/min. His weight is 3 kg (4th percentile) compared with 3.5 kg at birth (45th percentile). On physical exam, he is jaundiced with an enlarged liver and spleen. He does not appear to respond to visual stimuli, and further examination reveals bilateral clouding of the lens. Which of the following interventions could have avoided this patient's symptoms? \newline
\textbf{Options:} A. Avoiding fruit juice and sweetened foods; B. Changing to a soy-based formula; C. Providing imiglucerase enzyme replacement; D. Removing phenylalanine from maternal diet during pregnancy; E. Vitamin B\textsubscript{6} supplementation. \newline
\textbf{Correct Answer:} B (Changing to a soy-based formula). \newline
\textbf{Clinical Explanation:} 
This patient who presents with failure to thrive, hepatosplenomegaly, and bilateral cataracts most likely has classic galactosemia. Patients with this disorder should avoid lactose-containing products by changing to a soy-based formula. Classic galactosemia is an autosomal recessive defect in galactose-1-phosphate uridyltransferase. This enzyme is involved in the conversion of galactose to glucose, and a deficiency of this enzyme results in the accumulation of galactose 1-phosphate in the liver, kidney, and brain. This metabolite acts as a phosphate sink, meaning that it traps all free phosphate in the cytosol and inhibits the formation of other phosphate-dependent metabolites such as adenosine triphosphate. This results in failure to thrive, vomiting, lethargy, and hepatosplenomegaly after ingestion of galactose-containing products such as milk. Patients will also develop bilateral cataracts if the deficit is not detected in the first few weeks after birth. Avoiding galactose by changing to a soy-based formula will avoid the complications of this disorder. Turck discusses using soy protein for infant feeding. The author notes that there are safety concerns with regards to the high phyto-estrogenic isoflavone content of these formulas. The author recommends that despite these safety concerns, these formulas should still be used in patients with classic galactosemia.
} \\
\midrule
\multicolumn{3}{p{\linewidth}}{
\textbf{MedAgents expert analyses (5 domains).} \newline
\textbf{Pediatrics Expert:} 
This 4-week-old infant shows failure to thrive (weight decline from the 45th to the 4th percentile), poor feeding, tachycardia, and hepatosplenomegaly in the setting of persistent jaundice. The bilateral lens clouding and lack of visual tracking point to early-onset cataracts rather than isolated neonatal jaundice. The subacute time course after birth and the multisystem involvement (growth, liver, and eyes) strongly suggest a congenital metabolic disorder unmasked by routine feeding rather than an isolated infectious process. The most worrisome elements are the early age, progressive weight loss, and evolving liver disease, which together indicate an ongoing toxic exposure. \newline
\textbf{Medical Genetics Expert:} 
The triad of hepatosplenomegaly, jaundice, and neonatal cataracts is highly characteristic of classic galactosemia due to GALT deficiency. Without newborn screening or prenatal care, this diagnosis may be missed until symptoms appear after exposure to lactose-containing feeds. In galactosemia, excess galactose is phosphorylated to galactose-1-phosphate and also reduced to galactitol; these metabolites disrupt hepatic function and lens transparency. The key concern is that continued galactose intake rapidly leads to liver failure, sepsis (often \textit{E.~coli}), and neurodevelopmental injury, even though these outcomes are preventable with early dietary restriction. \newline
\textbf{Neonatology Expert:} 
A term infant with poor feeding, weight loss, and hepatosplenomegaly at 4 weeks raises alarm for a serious neonatal condition. The home birth and lack of prenatal care increase the likelihood of missed newborn screening. The constellation here---failure to thrive, cholestatic-appearing jaundice, and bilateral cataracts---is most consistent with a systemic inborn error of metabolism triggered postnatally by a specific nutrient in the diet. The most alarming feature is that every feed likely delivers the toxic substrate, so the clinical trajectory can deteriorate quickly unless the offending nutrient is removed. \newline
\textbf{Ophthalmology Expert:} 
Symmetric lens clouding in a neonate is classic for metabolic cataracts, particularly those caused by galactitol accumulation in galactosemia. Aldose reductase converts excess galactose into galactitol within the lens, creating an osmotic gradient that leads to lens fiber swelling and opacification. The absence of visual tracking indicates significant functional impairment. Importantly, early recognition and removal of galactose can prevent progression and, in some cases, partially reverse cataract formation. Unchecked exposure, however, risks permanent visual deficits. \newline
\textbf{Hepatology Expert:} 
Jaundice and hepatosplenomegaly at 4 weeks reflect true hepatic dysfunction, not physiologic jaundice. In classic galactosemia, galactose-1-phosphate accumulates in hepatocytes, leading to cholestasis, synthetic dysfunction, and enlargement of the liver and spleen. If dietary galactose is not eliminated, this process can progress to acute liver failure, coagulopathy, and sepsis. The most urgent issue is that the same nutrient (lactose/galactose) driving liver injury is still present in each feed, making prompt dietary modification central to both treatment and prevention.
}\\
\midrule
\textbf{Synthesized Report (v0):} & \textbf{Vote Result (all domains):} & \textbf{Revised Synthesized Report (v1):} \\
\textbf{Key Knowledge:} Classic galactosemia due to GALT deficiency explains the combination of failure to thrive, jaundice, hepatosplenomegaly, and neonatal cataracts in a 4-week-old infant who likely missed newborn metabolic screening. Ongoing ingestion of lactose-containing feeds results in accumulation of galactose-1-phosphate in the liver and galactitol in the lens. Early dietary intervention that removes the offending sugars can prevent hepatic failure and cataract progression. \newline
\textbf{Total Analysis (v0):} 
Integrating the experts' reports, the system concludes that this infant's presentation is best accounted for by a galactose-processing defect leading to toxic accumulation of galactose metabolites. Because both galactose and other simple sugars can place metabolic stress on the immature liver, a cautious preventive strategy is to broadly limit sugar exposure. Accordingly, the initial synthesis recommends \hlc{pink!60}{avoiding fruit juice and sweetened foods to reduce additional sugar load, and switching from standard milk or formula to a lactose-free, soy-based formula to eliminate dietary galactose.} This combined approach aims to minimize exposure to both galactose and other potentially harmful simple carbohydrates, thereby preventing the development of cataracts, hepatosplenomegaly, and failure to thrive in susceptible infants. 
&
\textbf{Pediatrics Expert:} Yes. The overall diagnosis (classic galactosemia) and emphasis on removing lactose/galactose are appropriate; the mention of fruit juice has little impact at 4 weeks but is not overtly harmful. \newline
\textbf{Medical Genetics Expert:} Yes. The core mechanism and the need to eliminate galactose are correctly described, though the focus on fructose-containing juices is somewhat tangential. \newline
\textbf{Neonatology Expert:} Yes. The synthesis captures that early dietary modification is preventive, although the practical relevance of fruit-juice avoidance is limited at this age. \newline
\textbf{Ophthalmology Expert:} \hlc{pink!60}{No. The cataracts here are specifically due to galactitol accumulation from galactose, not from generic sweetened foods. The report should emphasize that prevention hinges on eliminating galactose, not on broad sugar restriction.} \newline
\textbf{Hepatology Expert:} \hlc{pink!60}{No. The liver injury is driven by galactose-1-phosphate accumulation from lactose-containing feeds. The recommendation to avoid fruit juice is clinically irrelevant for a 4-week-old and distracts from the urgent need to remove galactose.} \newline
\textbf{Clinical Nutrition Expert:} \hlc{pink!60}{No. Fruit juice and sweetened foods are not part of a typical 4-week-old diet; the preventive intervention should focus solely on changing the infant's primary milk source to a lactose-free formula.} \newline
\textbf{Outcome:} Because several specialists disagree, MedAgents triggers a revision round, asking dissenting experts to propose edits that sharpen the causal link between galactose exposure and the preventive intervention.
&
\textbf{Incorporated Revision Advice:} Ophthalmology emphasizes that cataracts arise from galactitol produced specifically from galactose, not general sugar intake. Hepatology and Clinical Nutrition stress that fruit juice is irrelevant at 4 weeks and that the key is immediate removal of galactose-containing feeds. \newline
\textbf{Total Analysis (v1):} 
After incorporating the revision advice, the updated synthesis focuses on the precise causal relationship between galactose exposure and organ damage. Classic galactosemia due to GALT deficiency leads to accumulation of galactose-1-phosphate in the liver and conversion of excess galactose to galactitol in the lens. These metabolites cause cholestatic liver disease, failure to thrive, and neonatal cataracts. Crucially, these complications are \emph{specifically triggered by continued ingestion of lactose (and thus galactose) in breast milk or standard formula}. Preventing this clinical picture does not require broad restriction of all sugars, nor is it meaningfully influenced by fruit juice in a 4-week-old infant. Instead, the central preventive measure is to \hlc{teal!20}{eliminate dietary galactose as soon as the disorder is recognized by switching the infant from breast milk or standard formula to a lactose-free, soy-based formula.} This intervention removes the toxic substrate, halts further accumulation of galactose metabolites, and can prevent or mitigate both hepatic injury and cataract formation. Alternative options such as avoiding fruit juice, using imiglucerase, restricting maternal phenylalanine, or providing vitamin B\textsubscript{6} do not address the underlying defect and would not have avoided this patient’s symptoms. \newline
\textbf{Final MedAgents Answer:} \hlc{teal!20}{B. Changing to a soy-based formula.}
\\
\bottomrule
\end{tabular}
\end{table*}
